DeepPrivacy: A Generative Adversarial Network for Face Anonymization

We propose a novel architecture which is able to automatically anonymize faces in images while retaining the original data distribution. We ensure total anonymization of all faces in an image by generating images exclusively on privacy-safe information. Our model is based on a conditional generative adversarial network, generating images considering the original pose and image background. The conditional information enables us to generate highly realistic faces with a seamless transition between the generated face and the existing background. Furthermore, we introduce a diverse dataset of human faces, including unconventional poses, occluded faces, and a vast variability in backgrounds. Finally, we present experimental results reflecting the capability of our model to anonymize images while preserving the data distribution, making the data suitable for further training of deep learning models. As far as we know, no other solution has been proposed that guarantees the anonymization of faces while generating realistic images.

==> discriminator_architecture.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{|cclc|}
        \hline
        \textbf{Discriminator} & Act &  Output shape & Params  \\
        \hline
        Input image + conditional Info & -- &   $6\times128\times128$ & -- \\
        Conv $1\times1$ & LReLU & $176\times128\times128$ & 1.2K \\ 
        Stack pose information & -- & $183\times128\times128$ & -- \\ 
        Conv $3\times3$ & LReLU & $176\times128\times128$ & 290K \\ 
        Conv $3\times3$ & LReLU & $360\times128\times128$ & 571K \\
        Downsample & -- & $360\times64\times64$ & -- \\        
        \hline
        Stack pose information & -- & $367\times64\times64$ & -- \\ 
        Conv $3\times3$ & LReLU & $360\times64\times64$ & 1.2M \\ 
        Conv $3\times3$ & LReLU & $720\times64\times64$ & 2.3M \\
        Downsample & -- & $720\times32\times32$ & -- \\
        \hline
        Stack pose information & -- & $727\times32\times32$ & -- \\ 
        Conv $3\times3$ & LReLU & $720\times32\times32$ & 4.7M \\
        Conv $3\times3$ & LReLU & $720\times32\times32$ & 4.7M \\ 
        Downsample & -- & $720\times16\times16$ & -- \\ 
        \hline
        Stack pose information & -- & $727\times16\times16$ & -- \\ 
        Conv $3\times3$ & LReLU & $720\times16\times16$ & 4.7M \\
        Conv $3\times3$ & LReLU & $720\times16\times16$ & 4.7M \\ 
        Downsample & -- & $720\times8\times8$ & -- \\
        \hline
        Stack pose information & -- & $519\times8\times8$ & -- \\ 
        Conv $3\times3$ & LReLU & $720\times8\times8$ & 4.7M \\
        Conv $3\times3$ & LReLU & $720\times8\times8$ & 4.7M \\ 
        Downsample & -- & $720\times8\times8$ & -- \\    
        \hline
        Stack pose information & -- & $727\times4\times4$ & -- \\ 
        Conv $3\times3$ & LReLU & $720\times4\times4$ & 4.7M \\
        Conv $4\times4$ & LReLU & $720\times1\times1$ & 8.3M \\ 
        Fully-connected & linear & $  1\times1\times1$ & 721\\
        \hline
        Total trainable parameters & & & \textbf{45.5M} \\
        \hline
        
        
    \end{tabular}
    \vspace{2mm}
    \caption{The wide discriminator that we use to generate $128x128$ images.}
    \label{tab:my_label}
\end{table}

